Wiggins: Detecting Valuable Information in Dynamic Networks Using Limited Resources

Detecting new information and events in a dynamic network by probing individual nodes has many practical applications: discovering new webpages, analyzing influence properties in network, and detecting failure propagation in electronic circuits or infections in public drinkable water systems. In practice, it is infeasible for anyone but the owner of the network (if existent) to monitor all nodes at all times. In this work we study the constrained setting when the observer can only probe a small set of nodes at each time step to check whether new pieces of information (items) have reached those nodes. We formally define the problem through an infinite time generating process that places new items in subsets of nodes according to an unknown probability distribution. Items have an exponentially decaying novelty, modeling their decreasing value. The observer uses a probing schedule (i.e., a probability distribution over the set of nodes) to choose, at each time step, a small set of nodes to check for new items. The goal is to compute a schedule that minimizes the average novelty of undetected items. We present an algorithm, WIGGINS, to compute the optimal schedule through convex optimization, and then show how it can be adapted when the parameters of the problem must be learned or change over time. We also present a scalable variant of WIGGINS for the MapReduce framework. The results of our experimental evaluation on real social networks demonstrate the practicality of our approach.

==> tex/back.introduction.tex <==
\section{Introduction}\label{sec:introduction}
An emerging trend in algorithmic stock trading is the use of automatic search through the Web, the blogosphere, and social networks for relevant information that can be used in fast trading, before it appears in the more popular news sites~\cite{Delaney2009,ALPHA2014,AlphaFlash,mitra2011handbook,latar2015robot}. Similarly, intelligence, business and politics analysts are scanning online sources for new information or rumors. While new items are often rebloged, retweeted and posted on a number of sites, the goal is to find the information, somewhere, as fast as possible before we gradually loose the interest in them. %There is no benefit in seeing more copies of the same news item, rumor, etc.

Such a search is an example of a fundamental search and detection problem in dynamic, distributed massive data repository.  Data is distributed among a large number of nodes, new items appear in individual nodes, and items may propagate (copied) to neighboring nodes on a physical or a virtual network.  The goal is to detect at least one copy of each new item as soon as possible. The search application can probe any node in the system, but it can only access and process a few nodes at a time. 
To minimize the time to find new items, the search application needs to optimize the schedule of probing nodes, taking into account (i) the way items get distributed among the nodes (to see where to probe), and (ii) how items' freshness (or relevance) decay over the time (to avoid the worthless probes).

% the likelihood of nodes to generate new items, to receive new items, to propagate items to other nodes, and how yet undiscovered items loose their impact/value over the time.

Another application that faces a similar search problem is processing security raw data (e.g. gathered security raw footages that need to be processed). Ideally, given limited resources compared to the huge size of the data, an schedule for processing (probing) different raw-dataset has to minimize the value of missing information (assuming newer information are more valuable than older ones).

To formally define our search problem, {\probname} we need the following definitions.

\begin{definition}[Generating System]
 Suppose $U=\set{1,\ldots,n}$ is a universal set of elements, $\F$ is a family of subsets of $U$, and $\pi:\F \rightarrow [0,1]$. We call the elements of $\F$ \emph{\ins} of $U$. A \emph{generating system} $\sys = (U, \F,\pi)$ is an infinite time system that at each time step generates a random sample $\S\subseteq\F$, such that a set $S\in \S$ is randomly chosen with probability $\pi(S)$. Thus, $\sys$ generates a sequence $\S_1,\S_2,\ldots$ where each $\S_t$ is a sample of {\ins}s generated at time $t$. An \emph{item} $i_{t,S}$ is a \emph{copy} of the {\ins} $\S$ generated at time $t$.
\end{definition}

\begin{definition}[Schedule]
 For a positive integer $c$, a \emph{$c$-schedule} for a generating system $\sys=(U,\F,\pi)$ is a probability distribution $\p$ over $U^c$. Probing via  a schedule $\p$ is an infinite process, such that at any time step, we choose (up to) $c$ nodes chosen randomly according to $\p$ to probe. We say an item $i_{t,S}$ is \emph{caught} at time $t'\geq t$, if $\p$ probes a node of $\S$ at time $t'$, for the first time after time $t$.
\end{definition}

\begin{definition}[Cost]
Suppose $\sys =(U,\F,\pi)$ is a generating system and $\theta\in[0,1]$ is the decaying factor. The \emph{freshness} of an \emph{uncaught} item $i_{t,S}$ at time $t'\geq t$ is $\theta^{t'-t}$. Define the \emph{load} of $\sys$ at time $t$, denoted by $L_\sys(t)$, as a r.v. that equals to the sum of the freshness of uncaught items at time $t$. The $\theta$-\emph{cost}, or \emph{cost} in short, of a schedule $\p$ is defined as $\E_{t}(L_\sys(t))$. We denote the cost of $\p$ by $\cost{\p}$.
% = \sum_{S\in\F}\frac{\pi(S)}{1-\theta(1-\p(S))}.$$
\end{definition}

\begin{definition}[\probname]
 The goal in a $(\theta,c)$-{\probname} ($(\theta,c)$-PHSP) for a generating system $\sys$ is to find  a $c$-schedule with the minimum $\theta$-cost. We call a schedule \emph{optimal} if it has the minimum cost.
\end{definition}

Note that in $(\theta,c)$-PHSP, the parameter $\theta$ tunes our interest in older items. For instance, if $\theta=0$ then each item will stays in the system only for one step as its freshness disappears immediately. So, ideally, a schedule should catch as many \emph{new items} (generated in the current time step) as possible (\ahmad{This can be viewed as a multi-arm bandit problem where each element $u\in U$ represents a bandit, and the score we get total freshness of the items that we catch by probing $u$}). In the other extreme, if $\theta=1$, an ideal schedule should consider all the items for catching, regardless of their age.

Although we introduced the $(\theta,c)$-PHSP as a search problem, it gives us a very general framework for asking ``social network'' problems, such as finding the most \emph{influential}~\cite{borgs2014maximizing,kempe} or the most \emph{central}~\cite{yoshida2014almost} set of nodes:
 

\begin{itemize}
 \item {\bf Influence Maximization:} Given a social social network $G=(U,E)$ and a cascade model for propagation on $G$, the goal is to find a set of $c$ nodes that maximizes the size of the cascade seeded at these nodes. In \cite{borgs2014maximizing} they introduced the notation of random hyper-edge, a random subset of nodes sampled according to a distribution $\pi'$. They showed that for a given set of nodes $N$, the influence of $N$, $\sigma(N)$, is
 \begin{equation}\label{eq:infmax}
\sigma(N) = n\cdot \pr_{S\sim \pi'} (N \cap S \neq \emptyset),
 \end{equation}
 where $n$ is the number of nodes in $G$. Thus, a set $N\subseteq U$ of size $c$ has the maximum influence if and only if it maximizes $\Pr_{S\sim \pi'}(N\cap S\neq \emptyset)$. 
 
 Now, let $\sys=(U,\F,\pi)$ be the generating system in which $\F$ is the family of all subsets of $U$ and $\forall S\in \F: \ \pi(S) = \pi'(S)$. Suppose $\p$ is an optimal $c$-schedule of the $(0,c)$-PHSP for $\sys$. Note that without loss of generality, since $\theta=0$, we can assume that $\p$ always  probes a \emph{fixed} set of $c$ nodes, $N$, that minimizes the total missing freshness, i.e., the total probability of the items that $\p$ does not catch at a time step; this is because after each step all the items are removed and the system resets. So, we have
 $$\cost{\p} = \min_{N'\subseteq U: |N'|=c} 1 - \Pr_{S\sim \pi'}(N'\cap S\neq \emptyset) = 1 - \Pr_{S\sim \pi'}(N\cap S\neq \emptyset),$$
 and thus, $\Pr_{S\sim \pi'}(N\cap S\neq \emptyset)$ is maximized and $N$ is a set of $c$ nodes with maximum influence. 
 Therefore, the Influence Maximization problem can be translated into a proper $(0,c)$-PHSP.
 
 
 \item {\bf Set Centrality Maximization\cite{yoshida2014almost}:} 
 In~\cite{yoshida2014almost} the problem of finding a set of $c$ nodes with maximum centrality was studied, for two different centrality measures (betweenness and coverage). Here, we see how finding a set (of size $c$) with maximum betweenness centrality can be presented as a $(0,c)$-PHSP (the results hold for coverage centrality as well using the proper hyper-edges introduced in~\cite{yoshida2014almost}).
 
 In a network $G=(U,E)$, the betweenness centrality of a set $N\subseteq U$ is defined as\footnote{In some other works, different normalizing factors are considered. However, without loss of generality we let the normalizing factor to be $\frac{1}{n(n-1)}$.}
 $$C(N) = \frac{1}{n(n-1)}\sum_{u,v\in V} \frac{\tau(u,v; N)}{\tau(u,v)}$$
 where $\tau(u,v)$ is the number of shortest path from $u$ to $v$, and $\tau(u,v;N)$ is the number of shortest path from $u$ to $v$ that pass any node in $N$. The goal is to find a set of $c$ nodes with maximum betweenness centrality. Suppose $\pi'$ is a distribution over the shortest paths of $G$, where each shortest path $P_{u,v}$ is chosen with probability $\frac{1}{n(n-1)\tau(u,v)}$. If $\texttt{in}(P)$ denotes the internal nodes of the path $P$, it has been shown~\cite{yoshida2014almost,mattoe?} the most central set of $c$ nodes is a set $N$ such that 
 $$N\in \argmax_{N'\subseteq U: |N'|=c} \pr_{P\in\pi'}(\texttt{in}(P)\cap N' \neq \emptyset).$$
 
 
Let $\F$ be the family of sets $S$ where each $S$ is the internal nodes of a shortest path in $G$, and define 
 $$\forall S\in\F : \ \pi(S)=\sum_{\text{shortest path} P: \texttt{in}(P)=S} \pi'(S).$$
Now, if $\sys=(U,\F,\pi)$ is a generating system, using a similar argument as above, we can assume that an optimal $c$-schedule for its $(0,c)$-PHSP probes a fixed set of $c$ nodes, $N$, that also has the maximum centrality.
\end{itemize}

% Obviously, the $c$-PHSP is an NP-hard problem as it reduces to other NP-hard problems (e.g., influence maximization). However, these reductions are to the cases where $\theta=0$ and general positive integer $c$. 
In this work, we focus on $(\theta,1)$-PHSPs. In the following sections, we first study the $(\theta,1)$-PHSPs and provide different methods for finding the optimal schedule. We also show how in a generating system $\sys=(U,\F,\pi)$ our method works even if we do not have access to $\F$ or $\pi$, using only the samples of {\ins}s generated by $\sys$. Next, we show the scalablity of our method in using the MapReduce framework. Finally, we apply our method to a variety of real networks, and the results of our experiments demonstrate the practicality and optimality of our solution. 

% $\theta \in (0,1)$ and $c=1$ (see Figure~\ref{fig:square}) and show that it is possible to find  an optimal probing schedule for $1$-PHSP in $\sys=(\F, \pi, \theta)$, efficiently, and without having any prior information on distribution of items, i.e., knowing $\pi$ is not assumed in our algorithm.


% \begin{figure}[h!]
%   \centering
%     \includegraphics[width=0.25\textwidth]{figures/square.pdf}
%  \caption{}
% \label{fig:square}
% \end{figure}

% Specifically, our goal is to provide an efficient tool for a user who does not have a prior information on the generation and distribution of items in the network. We focus on simple, memoryless probing schedules that are easy to compute and require minimum storage. Our solution consists of two major components. We first develop an efficient algorithm for computing a near optimal schedule. Then, using Hoeffding's inequality, we show prove having only to a family $\M$  of \emph{sampled} informed set gathered during a very short amount of time (during $O(\log(n))$ time intervals, where $n$ is the number of nodes), without having access to $\S$,  $\pi$, or the network topology, we are still able to apply our method accurately. 




==> tex/biblio.tex <==
\setlength{\bibsep}{2.0pt}
%\fontsize{9}{10.2}
%\selectfont
\begin{thebibliography}{41}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Agumbe~Suresh et~al.(2012)Agumbe~Suresh, Stoleru, Denton, Zechman, and
  Shihada]{AgumbeSuresh2012}
M.~Agumbe~Suresh, R.~Stoleru, R.~Denton, E.~Zechman, and B.~Shihada.
\newblock Towards optimal event detection and localization in acyclic flow
  networks.
\newblock ICDCN'12, 2012.


\bibitem[Boyd and Vandenberghe(2004)]{BoydV04}
S.~Boyd and L.~Vandenberghe.
\newblock \emph{Convex optimization}.
\newblock Cambridge university press, 2004.

\bibitem[Bright et~al.(2006)Bright, Gal, and
  Raschid]{adaptive-bright2006adaptive}
L.~Bright, A.~Gal, and L.~Raschid.
\newblock Adaptive pull-based policies for wide area data delivery.
\newblock \emph{ACM TODS}, 31\penalty0 (2):\penalty0 631--671, 2006.

\bibitem[Cataldi et~al.(2010)Cataldi, Di~Caro, and Schifanella]{Cataldi2010}
M.~Cataldi, L.~Di~Caro, and C.~Schifanella.
\newblock Emerging topic detection on {T}witter based on temporal and social
  terms evaluation.
\newblock MDMKDD'10, 2010.

\bibitem[Chen et~al.(2009)Chen, Wang, and Yang]{Chen2009}
W.~Chen, Y.~Wang, and S.~Yang.
\newblock Efficient influence maximization in social networks.
\newblock KDD'09, 2009.

\bibitem[Chen et~al.(2010)Chen, Wang, and Wang]{Chen2010}
W.~Chen, C.~Wang, and Y.~Wang.
\newblock Scalable influence maximization for prevalent viral marketing in
  large-scale social networks.
\newblock KDD'10, 2010.

\bibitem[Christakis and Fowler(2010)]{Christakis2010}
N.~A. Christakis and J.~H. Fowler.
\newblock {{S}ocial network sensors for early detection of contagious
  outbreaks}.
\newblock \emph{PLoS ONE}, 5\penalty0 (9):\penalty0 e12948, 2010.

\bibitem[Dasgupta et~al.(2007)Dasgupta, Ghosh, Kumar, Olston, Pandey, and
  Tomkins]{dasgupta2007discoverability}
A.~Dasgupta, A.~Ghosh, R.~Kumar, C.~Olston, S.~Pandey, and A.~Tomkins.
\newblock The discoverability of the web.
\newblock WWW'07, 2007.

\bibitem[Dean and Ghemawat(2008)]{dean2008mapreduce}
J.~Dean and S.~Ghemawat.
\newblock MapReduce: simplified data processing on large clusters.
\newblock \emph{CACM}, 51\penalty0 (1):\penalty0 107--113,
  2008.

\bibitem[Delaney(2009)]{Delaney2009}
A.~Delaney.
\newblock \emph{The Growing Role of News in Trading Automation}, Oct. 2009.
\newblock
  \url{http://www.machinereadablenews.com/images/dl/Machine_Readable_News_and_Algorithmic_Trading.pdf}.

\bibitem[Golovin et~al.(2010)Golovin, Faulkner, and Krause]{Golovin2010}
D.~Golovin, M.~Faulkner, and A.~Krause.
\newblock Online distributed sensor selection.
\newblock IPSN'10, 2010.

\bibitem[Hardy(1991)]{Hardy91}
G.~H. Hardy.
\newblock \emph{Divergent series}, volume 334.
\newblock Am.~Math.~Soc., 1991.

\bibitem[Hart and Murray(2010)]{Hart2010}
W.~Hart and R.~Murray.
\newblock Review of sensor placement strategies for contamination warning
  systems in drinking water distribution systems.
\newblock \emph{J. Water Resources Planning and Manag.},
  136\penalty0 (6):\penalty0 611--619, 2010.
\newblock \doi{10.1061/(ASCE)WR.1943-5452.0000081}.

\bibitem[Hope(2015)]{wallstreet2015}
B.~Hope.
\newblock How computers trawl a sea of data for stock picks.
\newblock \emph{The Wall Street Journal}, Apr. 1st 2015.

\bibitem[Horincar et~al.(2014)Horincar, Amann, and
  Arti{\`e}res]{onlineRef-horincar2014online}
R.~Horincar, B.~Amann, and T.~Arti{\`e}res.
\newblock Online refresh strategies for content based feed aggregation.
\newblock \emph{World Wide Web}, 1--35, 2014.

\bibitem[Jung et~al.(2011)Jung, Heo, and Chen]{jung2011irie}
K.~Jung, W.~Heo, and W.~Chen.
\newblock {IRIE}: Scalable and robust influence maximization in social
  networks.
\newblock \emph{arXiv:1111.4795}, 2011.

\bibitem[Kempe et~al.(2003)Kempe, Kleinberg, and Tardos]{Kempe2003}
D.~Kempe, J.~Kleinberg, and E.~Tardos.
\newblock Maximizing the spread of influence through a social network.
\newblock KDD'03, 2003.

\bibitem[Kempe et~al.(2005)Kempe, Kleinberg, and Tardos]{Kempe2005}
D.~Kempe, J.~Kleinberg, and E.~Tardos.
\newblock Influential nodes in a diffusion model for social networks.
\newblock ICALP'05, 2005.

\bibitem[Krause and Guestrin(2011)]{Krause2011}
A.~Krause and C.~Guestrin.
\newblock Submodularity and its applications in optimized information
  gathering.
\newblock \emph{ACM TIST}, 2\penalty0 (4):\penalty0
  32:1--32:20, 2011.

\bibitem[Krause et~al.(2008)Krause, Leskovec, Guestrin, VanBriesen, and
  Faloutsos]{Krause2008}
A.~Krause, J.~Leskovec, C.~Guestrin, J.~VanBriesen, and C.~Faloutsos.
\newblock Efficient sensor placement optimization for securing large water
  distribution networks.
\newblock \emph{J.~Water Resources Planning and Manag.},
  134\penalty0 (6):\penalty0 516--526, 2008.

\bibitem[Krause et~al.(2009)Krause, Rajagopal, Gupta, and Guestrin]{Krause2009}
A.~Krause, R.~Rajagopal, A.~Gupta, and C.~Guestrin.
\newblock Simultaneous placement and scheduling of sensors.
\newblock IPSN'09, 2009.

\bibitem[Krause et~al.(2011)Krause, Guestrin, Gupta, and
  Kleinberg]{Krause2011Kleinberg}
A.~Krause, C.~Guestrin, A.~Gupta, and J.~Kleinberg.
\newblock Robust sensor placements at informative and communication-efficient
  locations.
\newblock \emph{ACM TSN}, 7\penalty0 (4):\penalty0 31:1--31:33, 2011.

\bibitem[Kuhlman et~al.(2013)Kuhlman, Tuli, Swarup, Marathe, and
  Ravi]{Kuhlman2013}
C.~J. Kuhlman, G.~Tuli, S.~Swarup, M.~V. Marathe, and S.~S. Ravi.
\newblock Blocking simple and complex contagion by edge removal.
\newblock ICDM'13, 2013.

\bibitem[Latar(2015)]{latar2015robot}
N.~L. Latar.
\newblock The robot journalist in the age of social physics: The end of human
  journalism?
\newblock In \emph{The New World of Transitioned Media}, 65--80.
  Springer, 2015.

\bibitem[Leskovec et~al.(2007)Leskovec, Krause, Guestrin, Faloutsos,
  VanBriesen, and Glance]{Leskovec2007}
J.~Leskovec, A.~Krause, C.~Guestrin, C.~Faloutsos, J.~M. VanBriesen, and N.~S.
  Glance.
\newblock Cost-effective outbreak detection in networks.
\newblock KDD'07, 2007.

\bibitem[Li and Tang(2011)]{Li2011}
A.~Li and L.~Tang.
\newblock The complexity and approximability of minimum contamination problems.
\newblock TAMC'11, 2001.

\bibitem[Mathioudakis and Koudas(2010)]{Mathioudakis2010}
M.~Mathioudakis and N.~Koudas.
\newblock Twittermonitor: Trend detection over the {T}witter stream.
\newblock SIGMOD'10, 2010.

\bibitem[McKinney(2011)]{McKinney2011}
W.~McKinney.
\newblock \emph{Structured Data Challenges in Finance and Statistics}, 2011.
\newblock
  \url{http://www.slideshare.net/wesm/structured-data-challenges-in-finance-and-statistics}.

\bibitem[Mitzenmacher and Upfal(2005)]{MitzenmacherU05}
M.~Mitzenmacher and E.~Upfal.
\newblock \emph{Probability and Computing: Randomized Algorithms and
  Probabilistic Analysis}.
\newblock Cambridge University Press, 2005.

\bibitem[Oita and Senellart(2011)]{survey-oita2011deriving}
M.~Oita and P.~Senellart.
\newblock Deriving dynamics of web pages: A survey.
\newblock TWAW'11, 2011.

\bibitem[Ostfeld et~al.(2008)Ostfeld, Uber, Salomons, Berry, Hart, Phillips,
  Watson, Dorini, Jonkergouw, Kapelan, di~Pierro, Khu, Savic, Eliades,
  Polycarpou, Ghimire, Barkdoll, Gueli, Huang, McBean, James, Krause, Leskovec,
  Isovitsch, Xu, Guestrin, VanBriesen, Small, Fischbeck, Preis, Propato,
  Piller, Trachtman, Wu, and Walski]{BWSN2008}
A.~Ostfeld et al.
\newblock The battle of the water sensor networks ({BWSN}): A design challenge
  for engineers and algorithms.
\newblock \emph{J.~Water Resources Planning and Manag.},
  134\penalty0 (6):\penalty0 556--568, 2008.

\bibitem[Sia et~al.(2007)Sia, Cho, and Cho]{fast-sia2007efficient}
K.~C. Sia, J.~Cho, and H.-K. Cho.
\newblock Efficient monitoring algorithm for fast news alerts.
\newblock \emph{Knowledge and Data Engineering, IEEE Transactions on},
  19\penalty0 (7):\penalty0 950--961, 2007.

\bibitem[Tang et~al.(2014)Tang, Xiao, and Shi]{tang2014influence}
Y.~Tang, X.~Xiao, and Y.~Shi.
\newblock Influence maximization: Near-optimal time complexity meets practical
  efficiency.
\newblock \emph{arXiv:1404.0900}, 2014.

\bibitem[Wolf et~al.(2002)Wolf, Squillante, Yu, Sethuraman, and
  Ozsen]{wolf2002optimal}
J.~L. Wolf, M.~S. Squillante, P.~Yu, J.~Sethuraman, and L.~Ozsen.
\newblock Optimal crawling strategies for web search engines.
\newblock WWW'02, 2002.
\end{thebibliography}


==> tex/theorems.tex <==
\section{Theorems}
\begin{theorem}
 For any graph, there is a unique optimal schedule.
\end{theorem}
\begin{proof}
 The cost of a schedule $p$ can be written as 
 $$\sum_{S}\pr{S}\frac{1}{\sum_{i\in S} p_i},$$
 which is a convex function. Now since the simplex $\Delta_{n-1}$, the set of all schedules, is convex, there is a unique optimal schedule $p^*$.
\end{proof}




For a schedule $p$ define $c(p) = (c_1(p), \ldots, c_n(p))$, where 
$$c_i(p) = \sum_{S:i\in S} \pr{S} \cdot \left(\frac{p_i}{\sum_{j\in S} p_j}\right)^2 = 
p_i^2 \sum_{S:i\in S} \pr{S} \cdot \frac{1}{\paran{\sum_{j\in S} p_j}^2}.
$$
Also, define a mapping $\tau$ from schedules to schedules as follows:
$$\frac{1}{Z}\paran{\sqrt{c_p^*(1)}, \ldots, \sqrt{c_p^*(n)}},$$
where $Z$ is the normalizing factor.

\begin{theorem}
 A schedule $p$ is optimal if and only if $\tau(p) = p$.
\end{theorem}
\begin{proof}
 Using Lagrange multipliers and uniqueness of the optimal schedule, $p$ is an optimal solution if and only if it is the only solution the the following system of equations, for variables $p_1, \ldots, p_n, \lambda$
 \begin{align}\label{eq:lagsystem}
 \sum_{S:i\in S} \pr{S}\frac{1}{\paran{\sum_{j\in S}p_j}^2} = \lambda, \ \forall i: 1\leq i \leq n.
 \end{align}
 
 
 On the other hand, $\tau(p) = p$ if and only if for every $i$, $1\leq i \leq n$:
 \begin{align}
  p_i &= \sqrt{c_i(p)/Z} = \frac{p_i}{\sqrt{Z}} \paran{\sum_{S:i\in S} \pr{S} \cdot \frac{1}{\paran{\sum_{j\in S} p_j}^2}}^{1/2} \\
  & \Leftrightarrow \sum_{S:i\in S} \pr{S}\frac{1}{\paran{\sum_{j\in S}p_j}^2} = Z,
 \end{align}
 which is a solution for the system of equations in (\ref{eq:lagsystem}), by letting $\lambda = Z$.
\end{proof}


